DART2: a robust multiple testing method to smartly leverage helpful or misleading ancillary information

In many applications of multiple testing, ancillary information is available, reflecting the hypothesis null or alternative status. Several methods have been developed to leverage this ancillary information to enhance testing power, typically requiring the ancillary information is helpful enough to ensure favorable performance. In this paper, we develop a robust and effective distance-assisted multiple testing procedure named DART2, designed to be powerful and robust regardless of the quality of ancillary information. When the ancillary information is helpful, DART2 can asymptotically control FDR while improving power; otherwise, DART2 can still control FDR and maintain power at least as high as ignoring the ancillary information. We demonstrated DART2's superior performance compared to existing methods through numerical studies under various settings. In addition, DART2 has been applied to a gene association study where we have shown its superior accuracy and robustness under two different types of ancillary information.

==> sections/acknowledgement.tex <==
\section*{Acknowledgment}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../manu"
%%% End:


==> sections/theory.tex <==
\section{Asymptotic Theory}
\label{sec:theory}
\begin{condition}\label{cond::sparse}
  Assume $m_1\leq r_2 m^{r_1} \leq r_2 n^{r_1/r_3}$ for some
  $r_1<(M^{L-1}+1)^{-1}$, $r_2>0$, and $r_3>0$.
\end{condition}

% Independent case, exact normal
Th1: FDR control in independent case, exact normal.\\
\begin{thm}\label{thm:indfdr}
Under condition~\ref{cond::sparse}, RDART controls the FDR at any pre-specified level $\alpha\in (0,1)$, i.e., $\lim_{m,n\to\infty}\FDR \leq \alpha$.
\end{thm}
% Independent case, asymptotic normal
Th2:....\\



% Weakly dependent case

\begin{condition}[Few self-dependent and hub nodes]\label{cond::wd}
Define
$\mA'=\{A\in\mA^{(L)}: |\Gamma_A|\geq\delta_{2m}=o(\sqrt{c_\md})\}$. Assume $|\mA'|=o(c_\md)$.
\end{condition}

Th2: Refined procedure, FDR control in weakly dependent case.

==> sections/unused.tex <==
=== Methods ===


From an asymptotic perspective, for $m$ hypothesis with $m \rightarrow \infty$, we require that the aggregation tree satisfies the following two conditions:
\begin{itemize}
  \item \textit{Condition 1: The aggregation tree has a finite number of Layers $L$.} This condition guarantees a sufficient number of node exist on the top layer to facilitate the asymptotic FDR control. Technically speaking, if the number of layers grows at a small rate of $m$ such as $\log (m)$, the asymptotic results still hold. For similicity purpose, we do not consider the grows rate of $L$ here.
  \item \textit{Condition 2: Every node has a finite number of children.}
  The screening stage mentioned in the following section dynamically tests the nodes in the aggregation tree. The hypotheses in rejected nodes are screened out and proceed to the refining stage. Nodes with more children may have a higher proportion of null hypotheses, decreasing rejection chances. 
  Thus, we want to restrict the number of children of each node. Specifically, we require that there exists a finite number $M$ so that $|\mC(A)|\leq M$. %For optimal performance, we recommend setting $M$ to 2.
\end{itemize}

Let the test statistic of hypothesis $i$ be $T_i$. We assume that 
$$T_i\sim N(\theta_i,\sigma_i^2), \quad \text{with } \theta_i=\left\{\begin{array}{lc}\leq 0&i\in\Omega_0;\\>0&i\in\Omega_1.\end{array}\right.$$ 
While more relaxed distribution assumptions for $T_i$ can be performed for RDART to ensure its asymptotic theoretical properties, for simplicity in , we will assume the Gaussian distribution for $T_i$ in the main text. See DART \citep{li2023dart} for possible relaxiations on $T_i$'s distributions.


The sensitivity, also named as power, is defined as
\begin{equation*}
\text{Sensitivity}=\frac{|\mR\cap\Omega_1|}{|\Omega_1|}
\end{equation*}
